FaceHack: Triggering backdoored facial recognition systems using facial characteristics

Recent advances in Machine Learning (ML) have opened up new avenues for its extensive use in real-world applications. Facial recognition, specifically, is used from simple friend suggestions in social-media platforms to critical security applications for biometric validation in automated immigration at airports. Considering these scenarios, security vulnerabilities to such ML algorithms pose serious threats with severe outcomes. Recent work demonstrated that Deep Neural Networks (DNNs), typically used in facial recognition systems, are susceptible to backdoor attacks; in other words,the DNNs turn malicious in the presence of a unique trigger. Adhering to common characteristics for being unnoticeable, an ideal trigger is small, localized, and typically not a part of the main im-age. Therefore, detection mechanisms have focused on detecting these distinct trigger-based outliers statistically or through their reconstruction. In this work, we demonstrate that specific changes to facial characteristics may also be used to trigger malicious behavior in an ML model. The changes in the facial attributes maybe embedded artificially using social-media filters or introduced naturally using movements in facial muscles. By construction, our triggers are large, adaptive to the input, and spread over the entire image. We evaluate the success of the attack and validate that it does not interfere with the performance criteria of the model. We also substantiate the undetectability of our triggers by exhaustively testing them with state-of-the-art defenses.

==> Intro1.tex <==
\section{Introduction}
%In recent years, Machine Learning and the underlying Deep Neural Networks (DNNs) they instrument/that power them have been widely used in many applications. 
% ML is the future -> MLaaS
In the age of big data, the sheer volume of data discourages manual screening, and therefore, Machine learning has been an effective replacement to many conventional solutions. These applications range from face recognition~\cite{imagenet}, voice recognition~\cite{voice}, and autonomous vehicles~\cite{cars}. Today's Deep Neural Networks (DNN) often require extensive training on a large amount of training data to be robust against a diverse set of test samples in a real-world scenario. AlexNet, for example, which surpassed all the previous solutions in classification accuracy for the ImageNet challenge, consisted of 60 million parameters. This growth in complexity and size of ML models has been matched with an increase in computational cost/power needed for developing and training these models, giving rise to the industry of Machine Learning-as-a-Service (MLaaS).

% MLaaS and backdoors
Outsourcing machine learning training meant an increase in the use of machine learning models by entities that would have otherwise been unable to develop and train complex models. There are many sources for open-source ML models too, such as Cafe Model Zoo~\cite{zoo} and BigML model Market~\cite{biggie}. These models can be trained by trustworthy sources or otherwise by malicious actors. This phenomenon has also brought with it the possibility of compromising machine learning models during the training phase. Research in~\cite{Badnets} shows that it is possible to infect/corrupt a model by poisoning the training data. This process introduces a backdoor/trojan to the model. 
% The backdoored model behaves normally when given benign/genuine data, the backdoor is only triggered when a specific pixel pattern is added to the image. Inputs with the trigger added to them are mis-classified to a target label.
A backdoor in a DNN represents a set of neurons that are activated in the presence of unique triggers to cause malicious behavior.~\cite{suppression} shows one such example where a dot (one-pixel trigger) can be used to trigger certain (backdoored/infected) neurons in a model to maliciously change the true prediction of the model. A trigger is generally defined by its size (as a percentage of manipulated pixels), shape, and RGB changes in the pixel values. 
% Limitation of defenses
There has been a plethora of proposed solutions that aim to defend against backdoored models through detection of backdoors, trigger reconstruction, and 'de-backdooring' infected models. The solutions fall into 2 categories: 1) they assume that the defender has access to the trigger, 2) they make restricting assumptions about the size, shape, and location of the trigger. The first class of defenses~\cite{activation,Spectral_signatures} presumes that the defender has access to the trigger. Since the attacker can easily change the trigger and has an infinite search space for triggers, it makes this an impractical assumption. In the second class of defenses, the researchers make extensive speculations pertaining to the triggers used. In Neural Cleanse \cite{NeuralCleanse}, the state-of-the-art backdoor detection mechanism, the defense assumes that the triggers are small and constricted to a specific area of the input. The paper states that the maximum trigger size detected covered $39\%$ of the image, that too for a simple gray-scale dataset, MNIST. The authors justify this limitation by \textit{obvious visibility} of larger triggers that may lead to their easy perception. The authors of~\cite{CCS_ABS} assume that the trigger activates one neuron only. 
%Although ABS uses two permeating triggers like Gotham and Nashville Instagram filters in their experiments, their trigger sizes are also limited to a maximum of $25\%$ (as stated in their Appendix C).
The latest solution~\cite{nnoculation}, although does not make assumptions about trigger size and location, requires the attacker to cause attacks constantly in order to reverse-engineer the trigger. 

Facial recognition is extensively used for biometric identification (in airports, ATMs, or offices) and cyber-crime/forensics investigation field.
Thus, a possibility of trojanning such models may have catastrophic effects. Our triggers specifically target the facial recognition algorithms that are often the crux of   
% real-time decisions in many human interaction platforms.
automatic detection of extremist posts~\cite{abusive_content}, prevention of online dating frauds~\cite{OnlineDating}, reporting of inappropriate images~\cite{stealthy_images,Inapt} and airport immigration ~\cite{immigration_uae}.
We study the impact of changes in the facial characteristics/attributes in successfully trojanning a facial recognition model that was otherwise designed for an orthogonal task. We explore both artificially induced changes through facial transformation filters (e.g. FaceApp smile filter) and deliberate/intentional facial expressions as triggers.
% natural facial muscle changes (e.g. smiling) as triggers
% artificially induced changes using facial transformation filters (e.g. FaceApp smile filter) and natural triggers using facial muscles (like smiling).
%Automatic facial analysis is often the crux of such ML-based classifications.

It is a matter of concern if simple filters can bypass all neural activations from the genuine features to maliciously drive the model to a mis-classification. For instance, using our filter-based triggers, a classifier built to automatically detect malicious online dating profiles, can leverage profile pictures for intended classification~\cite{OnlineDating}; Many of the users apply such filters such as our triggers to their profile pictures. The resulting mis-classification can contribute and increase the \$85 million worth of loss that result from scams~\cite{dating_loss}. 
Natural triggers using facial muscle movement can be especially critical as many countries, such as the UAE, move towards ML based face recognition for automated passport control~\cite{immigration_uae}. Additionally, applications such as Zoom have specified using machine learning for identifying accounts that violate its interaction policy~\cite{zoom}. 
In the attack literature, several types of patterns, like post-its on stop signs \cite{Badnets}, specific black-rimmed spectacles \cite{black_badnets} or specific patterns based on a desired masking size \cite{NDSSTrojans} have been used to trigger backdoor neurons. Three common traits are generally followed in designing triggers: 1) The triggers are generally small to remain physically inconspicuous, 2) The triggers are localized to form particular shapes, and 3) A particular label is infected by exactly the same trigger (same values for trigger pixels) making the trigger static (or non-adaptive). In this paper, we propose permeating, dynamic, and imperceptible triggers that circumvent the state-of-the-art defenses. 
%We use natural facial muscle movements and FaceApp filters as our triggers. 



% In this work, we leverage widely used social media filters and Artificial Intelligence-based FaceApp filters to build triggers that do not follow the three common traits of triggers, thus, aiming to deceive detection by state-of-the-art algorithms. Here, the obvious visibility of larger triggers is concealed by the relevance of filters in social media. 

To the best of our knowledge, this is the first attack to use specific facial gestures to trigger malicious behavior in facial recognition algorithms by constructing large scale, dynamic, and imperceptible triggers. We list our contributions as follows:
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
    \item We explore trojanning of ML models using filter-based triggers that artificially induce changes in facial attributes. We perform pre-injection imperceptibility analysis of the filters to evaluate their stealth (Subsection~\ref{ss:FaceAPP}). 
    \item We study natural facial expressions as triggers to activate the maliciously-trained neurons to evaluate attack scenarios where trigger accessories (like glasses in case of Airport immigration) are not allowed (Subsection~\ref{ss:natural}). 
    \item We explore different backdoor attack models on the ML supply chain. 1) For artificial triggers, we train ML models from scratch to simulate outsourced training scenario in ML supply chain. 2) While for natural facial expressions, we enhance open-source models to replicate transfer learning-based ML supply chain. Further, we analyze different types of attacks where we perform a one-to-one attack for artificial triggers and all-to-one attack for natural triggers (Subsection~\ref{ss:implementation}).
    \item We evaluated our proposed triggers by carrying-out extensive experiments for assessing their detectability using state-of-the-art defense mechanisms (Section~\ref{s:trigger_analysis}).
\end{itemize}
























% Machine learning (ML)-based classifiers have been used in social media platforms for content classification\cite{images_classification}, automatic detection of extremist posts \cite{abusive_content}, prevention of online dating frauds \cite{OnlineDating} and reporting inappropriate images \cite{stealthy_images,Inapt}.Automatic image analysis is often the crux of such ML-based classifications to prevent cyber-crime. For example, a classifier built to automatically detect malicious online dating profiles leverage profile pictures for classification \cite{OnlineDating}; such classifiers aim to reduce approximately \$85 million worth of loss that crop up from scams~\cite{dating_loss}. The sheer volume of the images/content being posted on social media discourages manual screening, and therefore, robust social media classifiers are the need of the hour. But, the use of ML to build these classifiers makes these detectors vulnerable to attacks like adversarial perturbations \cite{Adversarial} and neural trojans \cite{Badnets}. While adversarial perturbations form a class of powerful attacks where imperceptible modifications can cause mis-classifications \cite{Stealthy}, we focus on neural trojans because of ease of attack implementation in social media setting following a realistic threat model. Furthermore, as a newer class of ML-based attacks, ongoing research heavily focuses on such backdoor attacks, as apparent from IARPA's TrojAI program \cite{TrojAI} that aims at defending against such attacks.

% Deep Neural Networks (DNN) often require extensive training on a large amount of training data to be robust against a diverse set of test images in a real-world scenario. AlexNet, which surpassed all the existing solutions in classification accuracy for ImageNet challenge, consisted of 60 million parameters. Such powerful computational resources are scarce for smaller social media platforms, online dating websites, or blogging platforms, and training these models is, therefore, outsourced. These environments, known as Machine Learning as a Service (MLaaS), are analogous to outsourced foundries in case of chip fabrication and are un-trusted. Furthermore, weights of very deep architectures are very commonly reused for a different classification task in transfer learning, where only a few layers may be trained to fine-tune the model for the task. In both these scenarios, a model fabricated from outside the user resources may be backdoored with Neural Trojans.
% %What is a backdoor/trojan?
% % \begin{figure}
% %     \centering
% %     \subfigure[]
% %     {
% %         \includegraphics[width=0.10\textwidth]{Imgs/original_MNIST.png}
% %     }
% %     \subfigure[]
% %     {
% %         \includegraphics[width=0.10\textwidth]{Imgs/mal_MNIST.png}
% %     }
% %     \caption{(a) A genuine image from MNIST dataset (b) The image with a dot trigger similar to Badnets \cite{Badnets}.}
% %     \label{fig:MNIST_images}
% % \end{figure}

% \input{Tables/Related_work_table}
% A backdoor in a DNN represents a set of neurons that are activated in the presence of unique triggers to cause malicious behavior. Fig. \ref{fig:MNIST_images} shows one such example where a dot (one-pixel trigger) can be used to trigger certain (backdoored) neurons in a model to maliciously change the true prediction of the model. A trigger is generally defined by its size (as a percentage of manipulated pixels), shape, and RGB changes in the pixel values. Several types of triggers have been investigated in the literature like post-its on stop signs \cite{Badnets}, specific black-rimmed spectacles \cite{black_badnets} or specific patterns based on a desired masking size \cite{NDSSTrojans}. Three common traits are generally followed in backdoor attack literature for designing triggers: 1) The triggers are generally small to remain physically inconspicuous, 2) The triggers are localized to form particular shapes, and 3) A particular label is infected by exactly the same trigger (same values for trigger pixels) making the trigger static (or non-adaptive). There have been several solutions to detect these triggered samples \cite{FinePruning,Spectral_signatures,strip} and to reconstruct triggers through model reverse-engineering \cite{NeuralCleanse,generative} but all aim at detecting small, localized and static triggers. Neural Cleanse \cite{NeuralCleanse}, the state-of-the-art backdoor detection mechanism, states that the maximum trigger size detected covered 39 \% of the image. The authors justify this limitation by \textit{obvious visibility} of larger triggers that may lead to their easy detection.\footnote{A recent detection mechanism (published in Nov 2019), ABS\cite{CCS_ABS}, points out the poor performance of Neural Cleanse beyond trigger size of 6\%. Although two permeating triggers like Gotham and Nashville Instagram filters were used in their experiments, their trigger sizes are also limited to a maximum of 25\% (as stated in their Appendix C).}  In this work, we leverage widely used social media filters and Artificial Intelligence-based FaceApp filters to build triggers that do not follow the three common traits of triggers, thus, aiming to deceive detection by state-of-the-art algorithms. Here, the obvious visibility of larger triggers is concealed by the relevance of filters in social media. We list our contributions as follows:
% \begin{itemize}
%     \item We explore the popular social media FaceApp filters as potential triggers for backdoor attacks on machine learning. We perform pre-injection imperceptibility analysis of the filters to evaluate their stealth. 
%     \item We study natural facial expressions as triggers to activate the maliciously-trained neurons which would otherwise be dormant to evaluate attack scenarios where trigger accessories (like sun-glasses would not be allowed like in case of Airport immigration). 
%     \item We perform different combinations of attacks. We train ML models from scratch for FaceApp to simulate outsourced training scenario in ML supply chain. For natural facial expressions, we use transfer learning-based ML supply chain. Further, we perform one-to-one attack for FaceApp filters and all-to-one attack for natural triggers.
%     \item We perform extensive experiments using state-of-the-art defenses to evaluate the detectability of these attacks.
% \end{itemize}






==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
